Kitsune: Enabling Dataflow Execution on GPUs

State of art DL models are growing in size and complexity, with many modern models also increasing in heterogeneity of behavior. GPUs are still the dominant platform for DL applications, relying on a bulk-synchronous execution model which has many drawbacks and is ill-suited for the graph structure of DL applications. Many industry and academic works attempt to overcome these by employing vertical fusion but this approach still fails to realize three untapped opportunities: (1) the fact that many resources on the GPU are idle while only one operator executes due to temporal multiplexing of the SM; (2) lower energy from more intelligent on-chip data-movement which lends to higher performance in a power-provisioned environment. (3) inability to exploit hidden or reduction dimensions as a source of parallelism to ease pressure on batch size. This paper explores relatively uncharted territory, answering the following key question: Can modest adjustments to the current GPU architecture enable efficient dataflow execution, thereby circumventing the constraints of vertical fusion without necessitating a clean-slate architecture design. We develop Kitsune -- a set of primitives that enable dataflow execution on GPUs and an end-to-end compiler based on PyTorch Dynamo. Across 5 challenge applications, Kitsune can provide 1.3$\times$-2.3$\times$ and 1.1$\times$-2.4$\times$ performance improvement as well as 41%-98% and 16%-42% off-chip traffic reduction for inference and training, respectively.

==> figs/coverage.tex <==
\begin{tabular}{lrrrrrrrr}
\textbf{Application}               & \textbf{\begin{tabular}[c]{@{}r@{}}Batch \\ Size\end{tabular}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}\# Pipe / \\ \# Ops\end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}\% Ops \\ Pipelined\end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Pipe Lat. / \\ App Lat. (ms)\end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}\% Time \\ Pipelined\end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Subgraph / \\ App Traffic (MB)\end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}\% Traffic \\ Eliminated\end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Subgraph \\ Compute \%\end{tabular}}} \\ \hline

\multicolumn{1}{l|}{BERT (Tiny)}   & \multicolumn{1}{r|}{32,768}                                    & 10 / 36                                                                                  & \multicolumn{1}{r|}{28\%}                                                                & 0.82 / 3.29                                                                                       & \multicolumn{1}{r|}{25\%}                                                                 & 321 / 691                                                                                         & \multicolumn{1}{r|}{46\%}                                                                     & 11\%                                                                                        \\

\multicolumn{1}{l|}{DLRM}          & \multicolumn{1}{r|}{2,048}                                     & 16 / 21                                                                                  & \multicolumn{1}{r|}{76\%}                                                                & 0.34 / 0.71                                                                                       & \multicolumn{1}{r|}{48\%}                                                                 & 74 / 159                                                                                           & \multicolumn{1}{r|}{46\%}                                                                     & 7\%                                                                                         \\

\multicolumn{1}{l|}{MeshGraphNets} & \multicolumn{1}{r|}{1.3 M}                                     & 90 / 473                                                                                 & \multicolumn{1}{r|}{19\%}                                                                & 13.7 / 30.7                                                                                       & \multicolumn{1}{r|}{45\%}                                                                 & 864 K / 2.3 M                                                                                       & \multicolumn{1}{r|}{37\%}                                                                     & 11\%                                                                                        \\

\multicolumn{1}{l|}{NERF}          & \multicolumn{1}{r|}{65,536}                                    & 24 / 24                                                                                  & \multicolumn{1}{r|}{100\%}                                                               & 1.64 / 1.64                                                                                       & \multicolumn{1}{r|}{100\%}                                                                & 1,395 / 1,408                                                                                       & \multicolumn{1}{r|}{99\%}                                                                     & 16\%                                                                                        \\

\multicolumn{1}{l|}{GraphCast}     & \multicolumn{1}{r|}{40,962}                                    & 128 / 320                                                                                & \multicolumn{1}{r|}{40\%}                                                                & 137 / 298                                                                                         & \multicolumn{1}{r|}{46\%}                                                                 & 34 K / 129 K                                                                                       & \multicolumn{1}{r|}{27\%}                                                                     & 34\%                                                                                         \\ \hline
\end{tabular}

==> figs/dram.tex <==
% \begin{tabular}{lrrr}
% \multirow{2}{*}{\textbf{Subgraph}} & \multicolumn{1}{l}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Traffic \\ Reduction\end{tabular}}}} & \multicolumn{2}{c}{\textbf{Measured DRAM Util.}}                                   \\
%                                    & \multicolumn{1}{l}{}                                                                                                & \multicolumn{1}{l}{\textbf{Bulk-Sync.}} & \multicolumn{1}{l}{\textbf{Dataflow}} \\ \hline
% \multicolumn{1}{l|}{mgn\_mlp}  & 3.5$\times$                                                                                                                & 32.5\%                                  & 10.2\%                                \\
% \multicolumn{1}{l|}{dlrm\_bot}  & 15.3$\times$                                                                                                                & 5.0\%                                   & 0.5\%                                 \\
% \multicolumn{1}{l|}{dlrm\_top}  & 9.6$\times$                                                                                                                 & 8.1\%                                   & 1.9\%                                 \\
% \multicolumn{1}{l|}{bert\_ffn}     & 7.6$\times$                                                                                                                 & 24.7\%                                  & 2.4\%                                 \\
% \multicolumn{1}{l|}{nerf\_all}    & 116.1$\times$                                                                                                               & 33.3\%                                  & 0.9\%                                 \\
% \multicolumn{1}{l|}{gc\_nodes}     & 3.0$\times$                                                                                                                 & 33.1\%                                  & 7.7\%                                 \\
% \multicolumn{1}{l|}{gc\_edges}     & 2.5$\times$                                                                                                                 & 33.3\%                                  & 7.9\%                                 \\ \hline
% \end{tabular}
\begin{tabular}{lrrr}
\multirow{2}{*}{\textbf{Subgraph}} & \multicolumn{3}{c}{\textbf{DRAM Utilization}}                                                                        \\
                                   & \multicolumn{1}{l}{\textbf{Bulk-Sync.}} & \multicolumn{1}{l}{\textbf{\thethingsw{}}} & \multicolumn{1}{l}{\textbf{Ratio}} \\ \hline
\multicolumn{1}{l|}{\mgnmlp{}} & 32.5\% & 10.2\% & 3.2$\times$  \\
\multicolumn{1}{l|}{\dlrmbot{}} & 5.0\%  & 0.5\%  & 9.9$\times$  \\
\multicolumn{1}{l|}{\dlrmtop{}} & 8.1\%  & 1.9\%  & 4.3$\times$  \\
\multicolumn{1}{l|}{\bertffn{}}    & 24.7\% & 2.4\%  & 10.3$\times$ \\
\multicolumn{1}{l|}{\nerfall{}}   & 33.3\% & 0.9\%  & 39.1$\times$ \\
\multicolumn{1}{l|}{\gcnodes{}}    & 33.1\% & 7.7\%  & 4.3$\times$  \\
\multicolumn{1}{l|}{\gcedges{}}    & 33.3\% & 7.9\%  & 4.2$\times$  \\ \hline
\end{tabular}

==> figs/gemm-model.tex <==
\begin{tabular}{lrrr}
\textbf{Shape}                 & \multicolumn{1}{l}{\textbf{Cutlass \%}} & \multicolumn{1}{l}{\textbf{Model  \%}} & \multicolumn{1}{l}{\textbf{Model w/ Fast Qs \%}} \\ \hline
\multicolumn{1}{l|}{Mx128x128} & 22.96\%                                 & 33.10\%                                & 79.67\%                                          \\
\multicolumn{1}{l|}{Mx256x128} & 24.70\%                                 & 51.89\%                                & 95.76\%                                          \\ \hline
\end{tabular}


==> figs/gpus.tex <==
% \begin{tabular}{llrrr}
% \textbf{Model} & \textbf{Arch}               & \multicolumn{1}{l}{\textbf{TFLOP/s}} & \multicolumn{1}{l}{\textbf{GB/s}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}GFLOP\\ / GB\end{tabular}}} \\ \hline
% RTX 3090$^1$       & \multicolumn{1}{l|}{Ampere} & 142                                  & 936                               & 152                                                                               \\
% RTX A6000$^2$      & \multicolumn{1}{l|}{Ampere} & 309                                  & 768                               & 402                                                                               \\
% A100 80GB PCIe$^3$ & \multicolumn{1}{l|}{Ampere} & 312                                  & 1555                              & 201                                                                               \\ \hline
% RTX 4090$^1$       & \multicolumn{1}{l|}{Ada}    & 330                                  & 1008                              & 327                                                                               \\
% RTX 6000 Ada$^2$   & \multicolumn{1}{l|}{Ada}    & 720                                  & 960                               & 750                                                                               \\
% H100 80GB PCIe$^3$ & \multicolumn{1}{l|}{Hopper} & 756                                  & 2039                              & 371                                                                               \\ \hline
% \end{tabular}
% \begin{tabular}{lllrrrr}
% \textbf{} &
%   \textbf{} &
%   \textbf{} &
%   \multicolumn{1}{l}{\textbf{}} &
%   \multicolumn{1}{l}{\textbf{}} &
%   \multicolumn{2}{c}{\textbf{GM Speedup}} \\
% \textbf{} &
%   \textbf{Model} &
%   \textbf{TFLOP/s} &
%   \multicolumn{1}{l}{\textbf{GB/s}} &
%   \multicolumn{1}{l}{\textbf{GFLOP/GB}} &
%   \multicolumn{1}{l}{\textbf{SW Dataflow}} &
%   \multicolumn{1}{l}{\textbf{HW Dataflow}} \\ \hline
% \multirow{3}{*}{\rotatebox[origin=c]{90}{Ampere}}       & \multicolumn{1}{l|}{RTX 3090$^1$}        & 142 & 936  & 152 & 0.96$\times$ & 3.41$\times$ \\
%                               & \multicolumn{1}{l|}{RTX A6000$^2$}       & 309 & 768  & 402 & 2.54$\times$ & 9.06$\times$ \\
%                               & \multicolumn{1}{l|}{A100 80 GB PCIe$^3$} & 312 & 1555 & 201 & 1.26$\times$ & 4.52$\times$ \\ \hline
% \multirow{3}{*}{\rotatebox[origin=c]{90}{Ada \\ Hopper}} & \multicolumn{1}{l|}{RTX 4090$^1$}        & 330 & 1008 & 327 & 2.06$\times$ & 7.37$\times$ \\
%                               & \multicolumn{1}{l|}{RTX 6000 Ada$^2$}    & 720 & 960  & 750 & 4.73$\times$ & 16.9$\times$ \\
%                               & \multicolumn{1}{l|}{H100 80 GB PCIe$^3$} & 756 & 2039 & 371 & 2.34$\times$ & 8.35$\times$ \\ \hline
% \end{tabular}

\begin{tabular}{lllrrr}
\textbf{} &
  \textbf{} &
  \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}TFLOP/s, \\ GB/s\end{tabular}}} &
  \multicolumn{1}{l}{\textbf{Mach.}} &
  \multicolumn{2}{c}{\textbf{GM Speedup}} \\
\textbf{} &
  \textbf{Model} &
   &
  \multicolumn{1}{l}{\textbf{AMI}} &
  \multicolumn{1}{l}{\textbf{HW}} &
  \multicolumn{1}{l}{\textbf{SW}} \\ \hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{Ampere}} &
  \multicolumn{1}{l|}{3090$^1$} &
  142, 936 &
  152 &
  4.00$\times$ &
  0.96$\times$ \\
 &
  \multicolumn{1}{l|}{A6000$^2$} &
  309, 768 &
  402 &
  10.60$\times$ &
  2.54$\times$ \\
 &
  \multicolumn{1}{l|}{A100$^3$} &
  312, 1555 &
  201 &
  5.29$\times$ &
  1.26$\times$ \\ \hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{\begin{tabular}[c]{@{}l@{}}Ada / \\ Hopper\end{tabular}}} &
  \multicolumn{1}{l|}{4090$^1$} &
  330, 1008 &
  327 &
  8.63$\times$ &
  2.06$\times$ \\
 &
  \multicolumn{1}{l|}{6000 Ada$^2$} &
  720, 960 &
  750 &
  19.76$\times$ &
  4.73$\times$ \\
 &
  \multicolumn{1}{l|}{H100$^3$} &
  756, 2039 &
  371 &
  9.77$\times$ &
  2.34$\times$ \\ \hline
\end{tabular}
$^1$Desktop, 
$^2$Workstation, 
$^3$Server 


==> figs/load-balancing.tex <==
\begin{tabular}{llll}
\textbf{Operator}                         & \textbf{\begin{tabular}[c]{@{}l@{}}Bulk-Sync. \\ Latency (ms)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Initial\\ Ratio\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Tuned \\ Ratio\end{tabular}} \\ \hline
\multicolumn{1}{l|}{Linear(128x384)+ReLU} & 1.414                                                                       & 2                                                                & 1                                                               \\
\multicolumn{1}{l|}{Linear(128x128)+ReLU} & 1.077                                                                       & 2                                                                & 1                                                               \\
\multicolumn{1}{l|}{Linear(128x128)}      & 0.647                                                                       & 1                                                                & 1                                                               \\
\multicolumn{1}{l|}{LayerNorm}            & 2.556                                                                       & 4                                                                & 3                                                               \\ \hline
\end{tabular}


==> figs/power.tex <==
\begin{tabular}{llll}
\textbf{Freq (MHz)}       & \textbf{Bulk Sync.} & \textbf{Pipelined} & \textbf{Pipelined -NS} \\ \hline
\multicolumn{1}{l|}{1530} & 275                 & 269                & 275                    \\
\multicolumn{1}{l|}{825}  & 172                 & 140                & 140                    \\ \hline
\end{tabular}

==> figs/related-work.tex <==
\begin{tabular}{lllllllll}
\textbf{Architecture}                                                                                                  & \textbf{Cerebras} & \textbf{Graphcore} & \textbf{Wave} & \textbf{\begin{tabular}[c]{@{}l@{}}Matrix-\\ Engines\end{tabular}} & \textbf{SambaNova} & \textbf{\begin{tabular}[c]{@{}l@{}}Stream-\\ Dataflow\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}EyeRiss, \\ Simba, etc\end{tabular}} & \textbf{This Work}                                                  \\ \hline
\multicolumn{1}{l|}{Granularity of Dataflow}                                                                           & Tensor            & Tensor             & Scalar        & Scalar                                                             & Both?              & Scalar                                                              & Scalar                                                                  & Tensor                                                              \\
\multicolumn{1}{l|}{Mapping}                                                                                           & Static            & Static             & Static        & Dynamic                                                            & Static             & Dynamic                                                             &                                                                         & Dynamic                                                             \\
\multicolumn{1}{l|}{Synchronization}                                                                                   & Dynamic           & Static?            & Static?       & N/A                                                                & Static?            & Not shown                                                           & Static                                                                  & Dynamic                                                             \\
\multicolumn{1}{l|}{Data Orchestration}                                                                                & Compiler          & Compiler           & Compiler      & Programmer                                                         & Programmer?        & Not shown                                                           &                                                                         & Programmer                                                          \\
\multicolumn{1}{l|}{Load Balance}                                                                                      & Compiler          & Compiler           & Compiler      & N/A                                                                & Compiler           & Not handled                                                         &                                                                         & \begin{tabular}[c]{@{}l@{}}Compiler\\ (profile-guided)\end{tabular} \\
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}HW primitives \\ for dataflow integrable \\ into other hw\end{tabular}} & No                & No                 & No            & N/A                                                                & No                 & No                                                                  & No                                                                      & Yes                                                                 \\
\multicolumn{1}{l|}{DL Integration}                                                                                    & Poor              & Poor               & Poor          & Good                                                               & Poor               & Poor                                                                &                                                                         & Good                                                                \\ \hline
\end{tabular}

==> figs/table-patterns.tex <==
\begin{tabular}{p{1in}l}
\hline
\textbf{Pattern} & 
\textbf{Description} \\
\hline

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{tabular}[c]{@{}l@{}}
\includegraphics[width=1in]{figs/pat-elem-elem.pdf}
\end{tabular}
&
Elemwise + Elemwise
\\ \hline

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{tabular}[c]{@{}l@{}}
\includegraphics[width=1in]{figs/pat-lin-act.pdf}
\end{tabular}
&
Linear + Activation
\\ \hline

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{tabular}[c]{@{}l@{}}
\includegraphics[width=1in]{figs/pat-mlp.pdf}
\end{tabular}
&
Multi-Layer Perceptron
\\ \hline


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{tabular}[c]{@{}l@{}}
\includegraphics[width=1in]{figs/pat-attn.pdf}
\end{tabular}
&
Attention
\\ \hline

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{tabular}[c]{@{}l@{}}
\includegraphics[width=1in]{figs/pat-linear-bwd.pdf}
\end{tabular}
&
Linear Backprop.
\\ \hline

\end{tabular}

\begin{tabular}{c}
\includegraphics[width=2.5in]{figs/pat-legend.pdf}
\end{tabular}


==> figs/vert-kitsu-compare.tex <==
\begin{tabular}{llll}
\textbf{Application}                    & \textbf{Pass}            & \textbf{Vertical Fusion}                                      & \textbf{Kitsune Spatial Fusion} \\ \hline
% \multirow{2}{*}{\textbf{Pull-Push}}     & \multicolumn{1}{l|}{Fwd} &                                                               & Fully fused                     \\
                                        % & \multicolumn{1}{l|}{Bwd} &                                                               & Fully fused                     \\ \hline
\multirow{2}{*}{\textbf{BERT}}          & \multicolumn{1}{l|}{Fwd} & Linear+Add+Norm+Linear+GeLU & Fused attention, Fused FFN      \\
                                        & \multicolumn{1}{l|}{Bwd} & None                                                           & Fused LinearBWD                 \\ \hline
\multirow{2}{*}{\textbf{DLRM}}          & \multicolumn{1}{l|}{Fwd} & Linear+ReLU                                  & Fused Bottom MLP, Fused Top MLP \\
                                        & \multicolumn{1}{l|}{Bwd} & None                                                           & Fused LinearBWD                 \\ \hline
\multirow{2}{*}{\textbf{MeshGraphNets}} & \multicolumn{1}{l|}{Fwd} & Fully fused MLP                              & Fully fused MLP                       \\
                                        & \multicolumn{1}{l|}{Bwd} & None                                                           & Fused LinearBWD                 \\ \hline
\multirow{2}{*}{\textbf{NeRF}}          & \multicolumn{1}{l|}{Fwd} & Linear+ReLU                                  & Fully fused                     \\
                                        & \multicolumn{1}{l|}{Bwd} & None                                                           & Fused LinearBWD                 \\ \hline
\multirow{2}{*}{\textbf{GraphCast}}     & \multicolumn{1}{l|}{Fwd} & Linear+ReLU                                  & Fused MLP                       \\
                                        & \multicolumn{1}{l|}{Bwd} & None                                                           & Fused LinearBWD                 \\ \hline
\end{tabular}

==> figs/vert-kitsune-patterns.tex <==
\begin{tabular}{p{1in}lp{0.1in}p{0.1in}p{0.1in}p{0.1in}p{0.1in}p{0.1in}p{0.1in}p{0.1in}p{0.1in}p{0.1in}p{0.1in}p{0.1in}}
& 
& 
\multicolumn{4}{c}{\textbf{AStitch}} & 
\multicolumn{4}{c}{\textbf{Welder}} &
\multicolumn{4}{c}{\textbf{\thething{}}} \\
\textbf{Pattern} & 
\textbf{Description}  & 
\Circled{1} & \Circled{2} & \Circled{3} & \Circled{4} &
\Circled{1} & \Circled{2} & \Circled{3} & \Circled{4} &
\Circled{1} & \Circled{2} & \Circled{3} & \Circled{4} \\
\hline

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{tabular}[c]{@{}l@{}}
\includegraphics[width=1in]{figs/pat-elem-elem.pdf}
\end{tabular}
&
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Elemwise +\\ Elemwise\end{tabular}}
&
Yes & No & No & \multicolumn{1}{l|}{N/A} &
Yes & No & No & \multicolumn{1}{l|}{N/A} &
Yes & No & Yes & \multicolumn{1}{l}{N/A}
\\ \hline

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{tabular}[c]{@{}l@{}}
\includegraphics[width=1in]{figs/pat-lin-act.pdf}
\end{tabular}
&
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Linear +\\ Activation\end{tabular}} 
& 
No & No & No & \multicolumn{1}{l|}{No} &
No & No & No & \multicolumn{1}{l|}{No} &
Yes & Yes & Yes & \multicolumn{1}{l}{Yes}
\\ \hline

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{tabular}[c]{@{}l@{}}
\includegraphics[width=1in]{figs/pat-mlp.pdf}
\end{tabular}
&
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Multi-Layer \\ Perceptron\end{tabular}} 
& 
No & No & No & \multicolumn{1}{l|}{No} &
No & No & No & \multicolumn{1}{l|}{No} &
Yes & Yes & Yes & \multicolumn{1}{l}{Yes}
\\ \hline


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{tabular}[c]{@{}l@{}}
\includegraphics[width=1in]{figs/pat-attn.pdf}
\end{tabular}
&
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Attention\end{tabular}} 
& 
No & No & No & \multicolumn{1}{l|}{No} &
No & No & No & \multicolumn{1}{l|}{No} &
Yes & Yes & Yes & \multicolumn{1}{l}{Yes}
\\ \hline

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{tabular}[c]{@{}l@{}}
\includegraphics[width=1in]{figs/pat-linear-bwd.pdf}
\end{tabular}
&
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Linear\\ Backprop.\end{tabular}} 
& 
No & No & No & \multicolumn{1}{l|}{No} &
No & No & No & \multicolumn{1}{l|}{No} &
Yes & Yes & Yes & \multicolumn{1}{l}{Yes}
\\ \hline

\end{tabular}
\begin{tabular}{ll}
\multirow{2}{*}{
\includegraphics[width=1in]{figs/pat-legend.pdf}
} & $^1$Naive overlap possible with large number of CTAs. \\
& $^2$Depends on size of intermediates and whether they will spill from on-chip storage. \\
& $^3$Fusing a subset of these may be possible. \\
\end{tabular}

